Learning Representations Robust to Group Shifts and Adversarial Examples

Despite the high performance achieved by deep neural networks on various tasks, extensive studies have demonstrated that small tweaks in the input could fail the model predictions. This issue of deep neural networks has led to a number of methods to improve model robustness, including adversarial training and distributionally robust optimization. Though both of these two methods are geared towards learning robust models, they have essentially different motivations: adversarial training attempts to train deep neural networks against perturbations, while distributional robust optimization aims at improving model performance on the most difficult "uncertain distributions". In this work, we propose an algorithm that combines adversarial training and group distribution robust optimization to improve robust representation learning. Experiments on three image benchmark datasets illustrate that the proposed method achieves superior results on robust metrics without sacrificing much of the standard measures.

==> figures/fig_example_cub.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[scale=0.55]{figures/Red_faced_Cormorant_0009_2782350115.jpg}
         \caption{Training example 1 ($y$~: waterbird; $attr$~: water background).}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[scale=0.3]{figures/Gadwall_0008_433365004.jpg}
         \caption{Training example 2 ($y$~: landbird; $attr$~: land background).}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[scale=0.3,trim=0cm 6cm 0cm 1cm, clip=true]{figures/Red_faced_Cormorant_0002_56199272.jpg}
         \caption{Test example ($y$~: waterbird; $attr$~: land background).}
     \end{subfigure}
        \caption{\textbf{Example of spurious attributes.} Note that the correlations \textit{water} or \textit{land} between bird type $y$ and background $attr$ (short for \textit{attribute}) does not hold at test time.}
        \label{fig:cub_example}
\end{figure*}

==> unused/table_v2.tex <==
\begin{table}
  \caption{Improvements on robust metrics}
  \label{tab_v2}
  \centering
  \begin{tabular}{llllllllll}
    \toprule
    \multirow{2}{*}{Dataset} & \multirow{2}{*}{Noise} &  \multicolumn{4}{c}{Avg Clean}\\
     \cmidrule{3-6}
     & & Std ERM & ERM AT & Std DRO & DRO ATT \\
    \midrule
    \multirow{2}{*}{CUB}    & Batch &   &   &  &  \\
                              & Group &   &   & &  \\
                              \hline
    \multirow{2}{*}{CIFAR10} & Batch  &   &   & & \\
                              & Group  &   &   & &  \\
                              \hline
    \multirow{2}{*}{CelebA} & Batch  &   &   & &  \\
                              & Group  &   &   & &  \\

    \bottomrule
  \end{tabular}
\end{table}

==> unused/table_v2_sample.tex <==
\begin{table}
  \caption{Improvements on robust metrics (CUB)}
  \label{tab_v2}
  \centering
  \begin{tabular}{llllllllll}
    \toprule
     \multirow{2}{*}{Dataset} & \multirow{2}{*}{Noise} &   \multicolumn{4}{c}{Avg Clean} & \multicolumn{4}{c}{Avg Clean} \\
     \cmidrule{3-6}\cmidrule{7-10}
     & & Std ERM & ERM AT & Std DRO & DRO AT & Std ERM & ERM AT & Std DRO & DRO AT \\
    \midrule
    \multirow{2}{*}{CUB}    & Batch &   &   &  &  &&&&\\
                              & Group &   &   & &  &&&&\\
                              \hline
    \multirow{2}{*}{CIFAR10} & Batch  &   &   & & &&&&\\
                              & Group  &   &   & &  &&&&\\
                              \hline
    \multirow{2}{*}{CelebA} & Batch  &   &   & &  &&&&\\
                              & Group  &   &   & &  &&&&\\

    \bottomrule
  \end{tabular}
\end{table}



==> unused/tsne_cub.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph1}
         % \caption{Std ERM}
         \label{cub_std_ERM}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph2}
         % \caption{Adv ERM}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph3}
         % \caption{Std DRO}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph3}
         % \caption{Adv DRO}
         \label{cub_adv_DRO}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph1}
         % \caption{Std ERM}
         \label{cub_std_ERM}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph2}
         % \caption{Adv ERM}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph3}
         % \caption{Std DRO}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph3}
         % \caption{Adv DRO}
         \label{cub_adv_DRO}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph1}
         % \caption{Std ERM}
         \label{cub_std_ERM}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph2}
         % \caption{Adv ERM}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph3}
         % \caption{Std DRO}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph3}
         % \caption{Adv DRO}
         \label{cub_adv_DRO}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph1}
         \caption{Std ERM}
         \label{cub_std_ERM}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph2}
         \caption{Adv ERM}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph3}
         \caption{Std DRO}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{graph3}
         \caption{Adv DRO}
         \label{cub_adv_DRO}
     \end{subfigure}
        \caption{tSNE plot of CUB for each group. From \ref{cub_std_ERM} to \ref{cub_adv_DRO}}
        \label{fig:tSNE_cub}
\end{figure}
